TrailBlazer: Trajectory Control for Diffusion-Based Video Generation

Within recent approaches to text-to-video (T2V) generation, achieving controllability in the synthesized video is often a challenge. Typically, this issue is addressed by providing low-level per-frame guidance in the form of edge maps, depth maps, or an existing video to be altered. However, the process of obtaining such guidance can be labor-intensive. This paper focuses on enhancing controllability in video synthesis by employing straightforward bounding boxes to guide the subject in various ways, all without the need for neural network training, finetuning, optimization at inference time, or the use of pre-existing videos. Our algorithm, TrailBlazer, is constructed upon a pre-trained (T2V) model, and easy to implement. The subject is directed by a bounding box through the proposed spatial and temporal attention map editing. Moreover, we introduce the concept of keyframing, allowing the subject trajectory and overall appearance to be guided by both a moving bounding box and corresponding prompts, without the need to provide a detailed mask. The method is efficient, with negligible additional computation relative to the underlying pre-trained model. Despite the simplicity of the bounding box guidance, the resulting motion is surprisingly natural, with emergent effects including perspective and movement toward the virtual camera as the box size increases.

==> source/6_code.tex <==
\newpage
\section{Code}

TrailBlazer is mostly developed using the open source library \textsf{diffusers}. The core of TrailBlazer is the attention processor, whose implementation is shown in \SecRef{sec:routine} below (see  \texttt{diffusers.models.attention\_processor.AttnProcessor}). In addition,  subject morphing is achieved by modifying the forward function in \texttt{diffusers.models.unet\_3d\_condition.UNet3DConditionModel} to allow interpolated prompt embeddings as conditioning. We omit irrelevant code in order to simplify this section.

\subsection{Fundamental}
\label{sec:fund}
The code snippets in this section illustrate how TrailBlazer employs 2D Gaussian weights to generate the injection attention in the spatial and temporal attention editing steps.


\begin{tiny}
\begin{minted}{python}
def get_weight_map(
    res: int, bbox_ratios: List[float], attention_probs: torch.tensor
) -> (torch.tensor, BoundingBox):
    """To get guassian weight map associated to specific dimension, normalized
    by the maximum of the current cross attention map

    Args:
        res(int): the resolution of this weight map
        bbox_ratios(List[float]): a list of four numbers for bbox
        attention_probs(torch.tensor): the cross attention map from the base class
    Returns:
        (torch.tensor, BoundingBox): the gaussian patch for injection and its bbox
    """
    bbox = BoundingBox(res, bbox_ratios)
    x = torch.linspace(0, bbox.height, bbox.height)
    y = torch.linspace(0, bbox.width, bbox.width)
    x, y = torch.meshgrid(x, y, indexing="ij")
    noise_patch = gaussian_2d(
        x,
        y,
        mx=int(bbox.height / 2.),
        my=int(bbox.width / 2.),
        sx=float(bbox.height),
        sy=float(bbox.width),
    )
    noise_patch.mul_(attention_probs.max())
    return noise_patch, bbox

\end{minted}
\end{tiny}



\begin{tiny}
\begin{minted}{python}
def localized_spatial_weight_map(
    attention_probs_4d: torch.tensor, token_inds, bboxes_per_frame: List[List[float]]
):
    """Using guassian 2d distribution to generate weight patch as described in
    the equation (1), (2) in our main text.

    Args:
        attention_probs_4d(torch.tensor): the cross attention in the shape of (#heads, height, width, 77)
        token_inds(List[int]): the set of prompt word and trailing indices from user
        bboxes_per_frame(List[float]): a list of bbox ratios at frame
    Returns:
        (torch.tensor): the weight map for spatial injection

    """
    dim = int(attention_probs_4d.size()[1])
    weight_map = torch.zeros_like(attention_probs_4d).half()
    attn_head_size = attention_probs_4d.shape[0] // len(bboxes_per_frame)
    for i in range(len(bboxes_per_frame)):
        weight_patch = (
            get_weight_map(
                res=dim,
                bbox_ratios=bboxes_per_frame[i],
                attention_probs=attention_probs_4d,
            )
            # to match dimension
            .unsqueeze(0)
            .unsqueeze(-1)
            .repeat(attn_head_size, 1, 1, len(token_inds))
        )
        b_idx = attn_head_size * i
        e_idx = attn_head_size * (i + 1)
        bbox.sliced_tensor_in_bbox(weight_map)[
            b_idx:e_idx, ..., token_inds
        ] = weight_patch
    return weight_map
\end{minted}
\end{tiny}





\begin{tiny}
\begin{minted}{python}

def localized_temporal_weight_map(
    attention_probs_5d: torch.tensor, bboxes_per_frame: List[List[float]]
):
    """To generate the gaussian weight map matching the temporal attention
    dimensions. The Sm(x,y) in the equation (3) in TrailBlazer main text.

    Args:
        attention_probs_5d(torch.tensor): the cross attention in the shape of (#heads, height, width, #frames, #frames)
        bboxes_per_frame(List[float]): a list of four numbers determining the bbox corners
    """
    dim = int(attention_probs_5d.size()[1])
    f = attention_probs_5d.shape[-1]
    max_val = attention_probs_5d.max()
    weight_map = torch.zeros_like(attention_probs_5d).half()
    def get_patch(
        i: int, j: int, bbox_at_frame: List[float], bboxes_per_frame: List[List[float]]
    ):
        """To calculate the weight patch with distance function desbribed in
        Sm(x,y) in the paper
        Args:
            i(int): frame index
            j(int): frame index
            bbox_at_frame(List[float]): list of four numbers for bbox
            bboxes_per_frame(List[List[float]]): all bboxes per frame
        Returns:
            (torch.tensor): the weight map for temporal injection
        """
        weight_map = (
            get_weight_map(
                res=dim,
                bbox_ratios=bboxes_per_frame,
                attention_probs=attention_probs_5d,
            )
            # NOTE: to match dimension at layer
            .unsqueeze(0).repeat(attention_probs_5d.shape[0], 1, 1)
        )
        noise_patch.mul_(attention_probs_5d.max())
        inv_noise_patch = noise_patch - noise_patch.max()
        # NOTE: distance is large when
        dist = (float(abs(j - i))) / len(bboxes_per_frame)
        final_patch = inv_noise_patch * dist + noise_patch * (1.0 - dist)
        return final_patch, bbox
    # NOTE: To form the weight patch for each pair of bboxes of frames
    for j in range(len(bboxes_per_frame)):
        for i in range(len(bboxes_per_frame)):
            patch_i, bbox_i = get_patch(bboxes_per_frame[i], i, j, bboxes_per_frame)
            patch_j, bbox_j = get_patch(bboxes_per_frame[j], i, j, bboxes_per_frame)
            bbox_i.sliced_tensor_in_bbox(weight_map)[..., i, j] = patch_i
            bbox_j.sliced_tensor_in_bbox(weight_map)[..., i, j] = patch_j

    return weight_map

\end{minted}
\end{tiny}

\subsection{Main routine}
\label{sec:routine}
\begin{tiny}
\begin{minted}{python}
class InjecterProcessor():
    """The similar implementation as in
    diffusers.models.attention_processor.AttnProcessor from the open source
    project diffusers

    """
    def __init__(
        self,
        bundle: BundleType,
        bbox_per_frame: List[BoundingBox],
        strengthen_scale: float = 0.0,
        weaken_scale: float = 1.0,
    ):
        super().__init__(bundle)
        self.strengthen_scale = strengthen_scale
        self.weaken_scale = weaken_scale
        self.bundle = bundle
        self.bbox_per_frame = bbox_per_frame

    def __call__(
        self,
        attn: diffusers.models.attention_processor.Attention,
        hidden_states: torch.tensor,
        encoder_hidden_states: torch.tensor,
    ):
        """ The caller of attention prosessor
        Args:
            attn(Attention): the attention with
            hidden_states(torch.tensor): the latents from previous layer
            encoder_hidden_states(torch.tensor): text condition embeddings
        Returns:
        """
        batch_size, sequence_length, _ = hidden_states.shape
        # NOTE: To Q,K,V from latent and embeddings
        query = attn.to_q(hidden_states)
        key = attn.to_k(encoder_hidden_states)
        value = attn.to_v(encoder_hidden_states)
        query = attn.head_to_batch_dim(query)
        key = attn.head_to_batch_dim(key)
        value = attn.head_to_batch_dim(value)
        attention_probs = attn.get_attention_scores(query, key)

        # NOTE: To modify the spatial cross attention
        if (
            attention_probs.shape[-1] == CrossAttnProcessorBase.MAX_LEN_CLIP_TOKENS
            and self.use_spatial_editing
        ):
            dim = int(np.sqrt(attention_probs.shape[1]))
            attention_probs_4d = attention_probs.view(
                attention_probs.shape[0], dim, dim, attention_probs.shape[-1]
            )
            #
            attention_probs_4d = self.dd_core(attention_probs_4d)
            attention_probs = attention_probs_4d.reshape(
                attention_probs_4d.shape[0], dim * dim, attention_probs_4d.shape[-1]
            )
        # NOTE: To modify temporal cross frame attention
        elif attention_probs.shape[-1] == self.num_frames and (self.use_temporal_editing):
            dim = int(np.sqrt(attention_probs.shape[0] // attn.heads))
            attention_probs_5d = attention_probs.view(
                attn.heads, dim, dim, self.num_frames, self.num_frames,
            )
            attention_probs_5d = self.dd_core(attention_probs_5d)
            attention_probs = attention_probs_5d.view(
                (attn.heads * dim * dim, self.num_frames, self.num_frames),
            )

        hidden_states = torch.bmm(attention_probs, value)
        hidden_states = attn.batch_to_head_dim(hidden_states)
        # linear projection
        hidden_states = attn.to_out[0](hidden_states)
        # dropout
        hidden_states = attn.to_out[1](hidden_states)
        return hidden_states

    def dd_core(self, attention_probs: torch.Tensor):
        """
        Args:
            attention_probs(torch.tensor): A tensor either in 4d or 5d to
                trigger spatial or temporal attention editing, respectively.
        Returns:
            (torch.tensor): modified attention map

        """
        attention_probs_modified = attention_probs.detach().clone()

        # NOTE: Spatial cross attention editing
        if len(attention_probs.size()) == 4:
            # NOTE: token_inds is for specific prompt word
            token_inds = self.bundle.get("token_inds")
            # NOTE: trailing_inds is generated by the length determined by user
            trailing_length = self.bundle.get("trailing_length")
            trailing_inds = list(
                range(self.len_prompt + 1, self.len_prompt + trailing_length + 1)
            )
            all_tokens_inds = list(set(token_inds).union(set(trailing_inds)))
            # NOTE: To generate stengthen mask Ss(x,y) in Equation (1)
            strengthen_map = localized_weight_map(
                attention_probs_modified,
                token_inds=all_tokens_inds,
                bbox_per_frame=self.bbox_per_frame,
            )
            # NOTE: To generate weakening mask Ws(x,y) in Equation (1)
            weaken_map = torch.ones_like(strengthen_map)
            zero_indices = torch.where(strengthen_map == 0)
            weaken_map[zero_indices] = self.weaken_scale
            # NOTE: weakening in Equation (2)
            attention_probs_modified[..., all_tokens_inds] *= weaken_map[
                ..., all_tokens_inds
            ]
            # NOTE: strengthen in Equation (2)
            attention_probs_modified[..., all_tokens_inds] += (
                self.strengthen_scale * strengthen_map[..., all_tokens_inds]
            )
        # NOTE: Temporal cross attention editing
        elif len(attention_probs.size()) == 5:
            # NOTE: To generate stengthen mask in Equation (3)
            strengthen_map = localized_temporal_weight_map(
                attention_probs_modified,
                bbox_per_frame=self.bbox_per_frame,
            )
            # NOTE: To generate weakening mask as in spatial attention
            weaken_map = torch.ones_like(strengthen_map)
            zero_indices = torch.where(strengthen_map == 0)
            weaken_map[zero_indices] = self.weaken_scale
            # NOTE: weakening in Equation (3)
            attention_probs_modified *= weaken_map
            # NOTE: strengthen in Equation (3)
            attention_probs_modified += self.strengthen_scale * strengthen_map

        return attention_probs_modified

\end{minted}
\end{tiny}

==> source/s6_note.tex <==
\newpage

\section{Internal Note}
\label{sec:note}

@kurt Why edit:
this issue $>$ these limitations: because the preceding sentence only mentions one limitation not several

\textbf{Kurt todo:}\\
// teaser figure: change deformation to "morphing"


JP todo:
update cheetah section

//say something about why T2V and PB are the only baselines.\\
//Boximator\\
//Direct-a-video Feb\\
//peekaboo negative attention offset\\

QUESTIONS

We use the pre-trained ZeroScope model [6] (which is a fine-tuned version of [44]) as our underlying model. //is modelscope ref correct

378 However, changing bbox size and the corresponding perspective effects are not shown in Peekaboo’s tiger example

a cheetah running with a fixed camera

230 A larger number of trailing indices set

REDUCE SPACE: 
//omit 392 artifacts are common in diffusion models

376  for example if the camera is approaching the car from the side, 

comparisons vs peekaboo
less blurry background.
their fid/fvd is better, but comes at the expense of not following the bbox, and motion artifacts like tiger fliping direction (as well, their background is often blurred.
also following a fast bbox can introduce motion blur which may hurt fid measures.

we tried 10 random seeds

what is FID-vid?\\
limitations "see sup for fourther discussions",\\
subject morphing in abstract\\
competing methods feet moving but not walking

Peekaboo paper says it can change bbox size, however their released code does not appear to handle this.

We adjusted our resolutin to theirs (576,320) because their code worked poorly on square images.


It has 16 pages while the page limit is 14 pages excluding references. The ECCV24 rule is here (link). I think the task is clear for this submission:

1) Table:
I realize we have a table already but small. I'll try to add some recent method with public code for comparison, such as Peekapoo, 
 
2) Models: 
We claim TrailBlazer can work for any video diffusion model that uses temporal attention. However, one CVPR review argued whether this is true or not (i think it is). I'll try to see if there's any public video model so we can compare with.

3) Story refactor:
The top issue from CVPR review is that they complain we are sort of copying DD paper here, including figures (e.g., pipeline?) and equations. I guess I can try to re-design all figures to look a bit different. But I need your help on the story refactoring if possible, saying the work is built on DD in terms of novelty.

(Do you think the current approach is too naive for the submission? I guess we could probably analyze the spatial/temporal cross-attn directly from the video diffusion model, and edit the current formulation from that aspect)

4) New references:
There are some papers that were recently released this year (e.g., Direct-a-Video, Boximitor, Motion-Zero, no provided code), or some papers we missed (e.g., Peekapoo). I will try to update the related work on this.

TODO:
\begin{itemize}

    \item Our method builds on previous work, primarily that of Directed Diffusion [19]. However, our work addresses a different problem, that of controlling position and trajectories in videos, which requires careful control of temporal cross-attention. In addition, our work discards the optimization algorithm used in [19].


    \item question about trailing maps when there is more than one bbox

    \item JP near 96-

    \item section 4.1 and fig5: 
\JP{question: looking at the text2video-zero results, it looks like the subject is moving from right to left. With the normal math convention that +x means going right, this would mean the motion vector should be (-8,0) rather than (8,0)?}

    \item check new description above eq2

    \item in eq2 $w_r$ are hyperparams? need a statement about what their values are. "The weights $w_r$ are set to 0.9 in our experiments..."

    \item abstract: natural motion
    
    \item supp (discuss): "The following attention module signature is incorporated into our spatial attention editing list, with varied attention resolutions", not clear what the editing list is

    \item supp I think the single-keyframe (astronaut) motion slide could go \emph{before} the multiple-keys(cat), since it seems like a simpler experiment

    \item supp (check, discuss on call): Fig14, I think the order is "left/right top/bottom" rather than "clockwise"

    \item supp question fig7.4(single keyframe) "undesirable entity generation" -- means multiple legs or multiple astronauts?

    \item supp I noticed two paragraphs that seem similar, such as this on the last page. ARe the two paragraphs before+after chatgpt?
    
We demonstrate the irregular trajectory determined by varied keyframe in \FigRef{fig:supp_irr_path}. The four experiments with the trajectory of zigzag (top-left), triangle (top-right), discontinuity (bottom-left), and the down-pointing triangle (bottom-right). All horse result showcases the fast speed running with motion blur. However, the results with turning points has limitation to show the horse turning around and creates the artifacts. E.g., the third frame of down-pointing triangle case, that the horse swaps its head and tail. We think it is somewhat expected because it is naturally that a horse is good at charging forward rather than turning around with high speed like the cat or dog. In summary, the consistency between the prompt, the timing and bboxes in the keyframe must be maintained to increase the result fidelity.

We illustrate the irregular trajectory determined by varied keyframes in \FigRef{fig:supp_irr_path}. The four experiments involve zigzag trajectory (top-left), triangle trajectory (top-right), discontinuous trajectory (bottom-left), and down-pointing triangle trajectory (bottom-right). All horse results showcase fast-speed running with motion blur. However, results with turning points have limitations in depicting the horse turning around and may generate artifacts. For example, in the third frame of the down-pointing triangle case, the horse appears to swap its head and tail. This is somewhat expected, as horses are naturally better at charging forward than executing high-speed turns, unlike cats or dogs. Notably, some results show the perspective (e.g., down-pointing triangle) that the horse charging to the camera and then moving away, similar to the previous experience in \FigRef{fig:supp_dyn_bbox}, and also the car/tiger example \FigRef{fig:main_dyn}. In summary, maintaining consistency between the prompt, timing, and bounding boxes in the keyframes is crucial for increasing result fidelity.

    \item  intro line 31 need a reference for fine-tuning of sd for video. (Dreambooth is for images only I think?)

    \item quantitative section, maybe a statemnt "Following the methodology introduced in [paper], we apply FVD, to [a sequence of still images]..."

    \item L100 "Notably, We extend the exploration from DD that the SD is first position the objects, then refine the results."  // needs to be re-inserted 

    \item question r.e. this:  boxdiff,multidiffusion} have addressed the layout-to-image (L2I) issue using few-shot learning. The limitation is it only allow to generate the subject that are part of the training. // still have a question here, but low priority

    \item L429(quant) "without the supported input prior." // what does it mean

% LOW PRIORITY ------------------

    \item L133 "weight and the specific representation describing the image", explain to me later

\end{itemize}


JP a couple small notes on changes:\\
\begin{itemize}
[attention] depicted->discussed [in detail in sec 3.2, 3.3].  Depicted is ok but often suggests that the explanation mostly uses a picture to explain. Sec3.2 is mostly text/math
\item
all information between these keyframes is linearly interpolate $\rightarrow$ the information in these keyframes is linearly interpolate: original version is understandable, but someone might feel that the "all" might include all information in the image, not just the bounding box
\end{itemize}



